Enhancing Zero-shot Counting via Language-guided Exemplar Learning

Recently, Class-Agnostic Counting (CAC) problem has garnered increasing attention owing to its intriguing generality and superior efficiency compared to Category-Specific Counting (CSC). This paper proposes a novel ExpressCount to enhance zero-shot object counting by delving deeply into language-guided exemplar learning. Specifically, the ExpressCount is comprised of an innovative Language-oriented Exemplar Perceptron and a downstream visual Zero-shot Counting pipeline. Thereinto, the perceptron hammers at exploiting accurate exemplar cues from collaborative language-vision signals by inheriting rich semantic priors from the prevailing pre-trained Large Language Models (LLMs), whereas the counting pipeline excels in mining fine-grained features through dual-branch and cross-attention schemes, contributing to the high-quality similarity learning. Apart from building a bridge between the LLM in vogue and the visual counting tasks, expression-guided exemplar estimation significantly advances zero-shot learning capabilities for counting instances with arbitrary classes. Moreover, devising a FSC-147-Express with annotations of meticulous linguistic expressions pioneers a new venue for developing and validating language-based counting models. Extensive experiments demonstrate the state-of-the-art performance of our ExpressCount, even showcasing the accuracy on par with partial CSC models.

==> 3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> 3_method__Wang_Mingjie_________________2023-11-14_.tex <==
\section{Methodology}
As depicted in Figure~\ref{fig:main}, \mj{the overall architecture of our ExpressCount is mainly comprised of \emph{a novel Language-oriented Exemplar Perceptron}, succeeded by a \emph{Zero-shot Object Counting} branch. Specifically, when presented a textual expression coupled with the target scene, our perceptron excels at parsing} \& comprehending the natural language with \mj{rich semantic priors}. \mj{On top of the derived exemplar cues, the subsequent dual-branch counter proceeds to infer the total number of instances with unseen categories. The pipeline of ``language parsing$\rightarrow$zero-shot counting" marries the counting framework with human-imitated ability.}
\vspace{-0.2cm}
\subsection{Language-oriented Exemplar Perceptron}
\mj{The pase a few years have witnessed the flourishing of Large-scale Language Models (LLMs)} in many visual problems, such as point cloud analysis~\cite{zhu2023pointclip} and  visual grounding~\cite{zhu2022seqtr}. \mj{Thanks to strong semantic priors, LLMs substantially advance the capabilities, such as intelligence and interaction, across various vision problems. Considering the backwardness of language-based priors in the field of object counting, we pioneer to learn sufficient exemplar hints (\eg location and scale) through the high-quality guidance of natural language.} In particular, a language-oriented exemplar perceptron is proposed to characterize exemplar information, including geometrics, scales and locations, \mj{by learning a mapping between textual expression and bounding box of target exemplar}. \mj{Concretely, the perceptron consists of} a \emph{Linguistic Encoder}, a \emph{Visual Encoder} and a \emph{Transformer-based Multi-modal Integration} module, which will be elaborated in the rest of this section. 

\vspace{-0.2cm}
\paragraph{Linguistic Encoding}{Taking a \mj{language expression/text prompt} $re_l$ as input, we \mj{first utilize the basic pre-trained BERT model~\cite{devlin2018bert}  to extract rich semantics from linguistic signals as a large amount of modern LLMs are evolved from the fundamental BERT. In specific, the extraction of linguistic representation is achieved by the sequence of} tokenization ($T_l$) and embedding ($E_l$) operations. Wherein, $T_l$ is responsible for converting every word from the given sentence into \mj{diverse tokenized features (tokens)} in the vocab, whereas $E_l$ \mj{units are built upon a set of transformer layers, aiming to capture high-level semantics from tokens.} Following the common practice of \mj{BERT-based models}, a \mj{randomly-generated} token \emph{[cls]} \mj{is introduced as the regression token and is concatenated with the tokenized features, } while a token \emph{[sep]} is placed at the end of the tokenized features. \mj{The amalgamated  token sequence is then fed into the embedding units to model the global relationships among local tokens. As the training of pre-trained LLM takes hundreds of millions of natural language instances into account, its generated embeddings effortlessly distil and encapsulate rich semantic priors from the input expressions. The calculation process can be denoted as} $F_l = E_l(T_l(re_l)) \in R^{D_l\times N_l}$, where $D_l$ and $N_l$ denotes the length and number of the language tokens, and are set to 768 and 20, respectively. For simplicity, the dimension of batch size is omitted in the presence of feature shapes.}

\vspace{-0.2cm}
\paragraph{Visual Encoding}
Although the ultra goal of the referring expression comprehension for counting in this work is to infer  location cues deriving from pure linguistic signals, the lack of spacial guidance degrades the learning quality. Inspired by the idea of stable diffusion-based image synthesis~\cite{rombach2022high}, we take a noisy dark image $x_i \in R^{3 \times H_l \times W_l}$ as the input of visual encoder, and force the holistic model to regress the target coordinates conditioned on the input expression $C(F_l|x_i)$. The  visual encoding workflow can be divided into shallow feature extraction and global semantics modeling. A pre-trained ResNet ($R_i$) is utilized here to extract shallow representations with locality-oriented semantics $f_{s} \in R^{2048\times \frac{H_l}{32} \times \frac{W_l}{32} }$, which is subsequently fed into a 1$\times$1 conv layer to compress the 2048 kernels into compact 256-channel features $f_{st} $. A sequence of transformer layers (256 width) $T_i$ with 8-head attention mechanisms are then configured to mine global semantics from $f_{st}$. Finally, the advanced visual embeddings are derived as $F_i = T_i(R_i(x_i)) \in R^{D_i\times N_i}$, where $D_i=256$ represents length of channel dimension whereas $N_i=\frac{H_l}{32}\times \frac{W_l}{32}$ denotes the token number.
\vspace{-0.2cm}
\paragraph{Transformer-based Multi-modal Integration}

%\begin{figure}[h]
%	\begin{center}
	%		\includegraphics[width=\linewidth]{LV.pdf}
	%	\end{center} 
%	\caption{The details of our proposed multi-modal integration pattern for location prediction from linguistic inputs.}
%	\label{fig:LV}
%\end{figure}

After obtaining the linguistic and visual embeddings separately, our method proceeds to integrate the text-vision sibling features for synthesizing the target bounding box. %Transformer has been widely used as the best paradigm to process multi-modal signals thanks to its higher flexibility and global modelling capability. 
A transformer-based fusion module is used here since Transformer's global modeling capability makes it the best paradigm for processing multi-modal signals. Specifically, a concatenation is performed on a learnable token $[Loc] \in R^{256\times 1}$ and text-vision embeddings [$Loc$, $F_l$, $F_i$] $\rightarrow$$F_{li} \in R^{256\times (1+N_l+N_i)}$. Then $F_{li}$ is fed into a sequence of 6 transformer layers to mix and characterize the multi-modal representations, thereby enriching the head token $[Loc]$ with plenty of  information content. A regression head consisting of ``three Linear Projections, one Sigmoid Function" is placed at the end of this unit to parse the $[Loc]$ and predict the box information with the shape of $(x,y,h,w)$. %To better understand the aforementioned procedure, we visualize the integration scheme in Figure~\ref{fig:LV}.
\vspace{-0.2cm}
\subsection{Zero-shot Object Counting}
%Human-imitated expression comprehension attempts to understand spatial distributions of objects and infer the possible location cues by assimilating easy-to-get natural language signals, which lays the foundation of the zero-shot counting in this paper. 
This section will present the details of our counts regressor, which involves cascaded \emph{Sibling Backbone and Cross-attention Matching.}
\vspace{-0.2cm}
\paragraph{Sibling Backbone}
Differing from the mainstream practices, we  devise a sibling backbone with two pre-trained ResNets for learned exemplar and the raw counting scene. This is motivated by the observation that receptive fields or semantics for exemplar and raw image should be discriminative (object details \& instance repetition). Given the bounding box $(x,y,h,w)$ and raw image $I\in R^{3\times H \times W}$, we crop and resize the exemplar patch $I_e \in R^{2048\times128\times128}$ from $I$ automatically, and feed them into the sibling ResNets $R_e$ and $R_I$ to calculate basic 2D features $F_e=R_e(I_e) \in R^{2048\times8\times8}$ and $F_I=R_I(I_I) \in R^{2048\times\frac{H}{16}\times \frac{W}{16}}$. 1$\times$1 conv operations are then imposed to reduce and align the channel dimension ($F_e\in R^{256\times8\times8}$ \& $F_I \in R^{256\times\frac{H}{16}\times \frac{W}{16}}$). To represent 1D global semantics from the exemplar feature, instead of using average global pooling (AVG), we delicately design a fine-grained extractor comprised of a sequence of ``Patch Spliting$\rightarrow$Linear Projection$\rightarrow$1$\times$1Conv". After processing, a vector $\hat{F_e}\in R^{1\times256}$ representing exemplar information is produced. 
\vspace{-0.2cm}
\paragraph{Cross-attention Matching}
After obtaining the fundamental  features ($\hat{F_e}$ and $F_I$) for the exemplar and raw images, our CAC model proceeds to regress the final counts through cross-attention matching learning. Considering the potential heterogeneity in semantic space, a cross-attention mechanism is proposed to recalibrate the feature conditioned on the other one, denoted as $CA(\hat{F_e}|F_I) \cup CA(F_I|\hat{F_e})$. Specifically, towards recalibrating $\hat{F_e}\in R^{1\times256}$, we take $F_I \in R^{256\times\frac{H}{16}\times \frac{W}{16}}$ as the input and then adopt operations ``Matrix Multiplication $M_1$, Linear Transformation $L_1$ and Sigmoid Function" to generate the weights $W_1\in R^{1\times256} =L_1(M_1(\alpha_1F_I,\alpha_2F_I)).Sigmoid()$, where $\alpha_1$ and $\alpha_2$ are the trainable balance factors. Simultaneously, the input $\hat{F_e} \in R^{1\times256}$ passes through the workflow of ``Linear Transformation $L_2$ and Sigmoid Function" to generate the weights $W_2\in R^{1\times256}=L_2(\hat{F_e}).Sigmoid()$. Finally, the re-calibrations are executed based on the learned weights, denoted as  $\hat{F_e}  = \hat{F_e}  \times W_1$ and $F_I = F_I \times W_2$, respectively.


\paragraph{Counting-specific Expression Generation}
\begin{figure}[h]
	\begin{center}
		\includegraphics[width=\linewidth]{expressgen.jpg}
	\end{center} 
	\caption{The coarse-to-fine generation procedure of the counting-specific referring expressions in FSC-147-Express.}
	\label{fig:expressgen}
\end{figure}

Albeit the flourishing of language-vision data for various vision tasks (\eg point clouds, text-to-image and visual grounding), the explorations of linguistic counting are scarce due to the lack of language-vision annotations, thereby seriously damaging the interaction and generalization abilities of counting models nowadays. To this end, we extend the most prevailing benchmark FSC-147 designed for zero-shot counting, and release an expression-equipped dateset, namely \emph{FSC-147-Express}. As depicted in Figure~\ref{fig:expressgen}, we carefully device a coarse-to-fine synthesize protocol of counting-specific referring expressions by virtue of distilling knowledge from the powerful LLMs (BLIP). For example, given a counting scene, high-level question prompts are first designed (\eg \emph{``What objects does this image include?"}) and executed to generate coarse expressions including main class types. After capturing the class information, we further use counting-specific prompting (\eg \emph{``How many donuts? Describe the [class] details."}) to generate the referring expression with fine-grained cues, such as quantifier (``a bunch of/a bowl of") and action (``holding"). It is interesting that our proposed protocol allows to introduce count priors (\ie \emph{``a bunch of" v.s. ``a pile of"}) into the linguistic signals. By doing so, our efforts may have a far-reaching influence on the transferability of counting models.


\paragraph{Objective Function}
The overall optimization of our ExpressCount goes in a hybrid directions of Referring Expression Comprehension and Zero-shot Counting learning. To force the sub-network of linguistic comprehension to regress accurate bounding boxes, following the common practices in object detection, we utilize $L_1$ distance as  supervisory signals $L_l$. Concretely, given the predicted location $E_p(x_p,y_p,h_p,w_p)$ and the ground truth of $E_g(x_g,y_g,h_g,w_g)$, the linguistic error is calculated as:
\begin{equation}\label{LE}
	L_l = \sum_{i=1}^{N}(|x_g-x_p)|+|y_g-y_p|+|h_g-h_p|+|w_g-w_p|),
\end{equation}
where $N$ indicates the batch size while $h_p/h_g$ and $w_p/w_g$ denote the heights and widths of bounding boxes, respectively. The counting loss $L_c$ is a sliding loss term to supervise the counting sub-network to produce precise instance counts. When obtaining the predicted and ground-truth counts $C_p$ and $C_g$, we derive the counting loss as $L_c = \sum_{i=1}^{N}(|C_g-C_p|)$.
%\begin{equation}\label{LC}
%L_c = \sum_{N}^{i=1}(|C_g-C_p|).
%\end{equation}



























==> sec/0_abstract.tex <==
\begin{abstract}
Unlike Category-Specific Counting (CSC) models, a Class-Agnostic Counting (CAC) approach possesses the capability to perform various tasks by understanding and adapting to diverse contexts. It can seamlessly count objects in different settings, be it cells in a biology slide, people in crowd images, or stars in a galaxy, without the need for extensive retraining.  
A novel architecture is proposed in this paper to further enhance CAC through steering zero-shot counting via referring expression comprehension. Specifically, our Expression Counting Network (\emph{ExpressCount}) attempts to infer exemplar cues by acquiring knowledge from linguistic signals. The learned explicit exemplars, together with the query scene, are then fed into the cascaded counting network to achieve higher-performance counts prediction. In particular, our proposed method embraces the merits of plug-and-play and generalized applicability. The linguistic-centered attribute further enables the bridging of  visual counting and other language-visual models. Additionally, extending FSC-147 (\emph{FSC-147-Express}) blazes a trail for testifying counting models' capacity of expression understanding by designing fine-grained referring expressions for each sample. Extensive experiments demonstrate that our method surpasses all current CAC approaches with state-of-the-art accuracy and is quantitatively on par with partial CSC models.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\begin{figure}[h]
	\begin{center}
		\includegraphics[width=\linewidth]{comp1.jpg}
	\end{center} 
	\caption{(a) The exemplar-reliant CAC models require the user-provided exemplars, which need heavy manual costs to specify object locations and hinder model's applicability; (b) Inchoate exemplar-free CAC hammers at learning exemplar cues in a self-perception manner, and tends to produce unsatisfactory results due to the lack of semantics priors.}
	\label{fig:comp1}
\end{figure}

During the past decade, the Category-Specific Counting (CSC) problem has been widely studied, resulting in a wide range of techniques that achieve stunning results, such as crowd counting~\cite{liang2023crowdclip,ranasinghe2023diffuse,song2021rethinking,li2018csrnet}, cells~\cite{khan2016deep}, fruits~\cite{rahnemoonfar2017deep} and vehicles~\cite{bui2020vehicle}. Albeit exhibiting promising values, their success requires the collection of massive annotations for unique object class (\eg  1.51 million dots for the JHU-CROWD++~\cite{sindagi2020jhu}). 
%extensively explores high-capacity models hammering at regressing people numbers across congested scenes, whereas several approaches make efforts to count object instances with other categories, such as 
To unburden the notorious labeling costs and widen the applicability of counting models, a train of Class-Agnostic Counting (CAC) models~\cite{chattopadhyay2017counting,lu2018class,yang2021class,ranjan2021learning,shi2022represent,ranjan2022exemplar,lin2022scale,you2023few,jiang2023clip, wang2023gcnet,xu2023zero}  draw increasing attention from the research community to subitize or count object instances dispersing across the whole input scenes with arbitrary classes. Wherein, most of them require high-quality  user-provided exemplars for features matching learning (see Figure~\ref{fig:comp1}(a)), which is intractable for some real-world applications, like underwater biological monitoring system, where objects in question are amorphous. 

More recently, researches are shifting to a more dramatic  paradigm with fully exemplar-free settings (\ie zero-shot counting) referred to as Exemplar-Free Counting (EFC)~\cite{ranjan2022exemplar,jiang2023clip, wang2023gcnet,xu2023zero}. Particularly, existing EFC models either mine underlying repetitive patterns from the image signals~\cite{ranjan2022exemplar,wang2023gcnet} (see Figure~\ref{fig:comp1}(b)), or turn to class name for increasing discriminability of objects~\cite{xu2023zero,jiang2023clip}. Although these efforts have been made to ease the unreasonable demand of human-annotated bounding boxes and attain reasonably good results, the following drawbacks impede their potential applicability:
\begin{figure}[t]
	\begin{center}
		\includegraphics[width=\linewidth]{comp2.jpg}
	\end{center} 
	\caption{Our proposed linguistics-centered protocol where the counter is capable of parsing human language and predicting accurate exemplars. } 
	\label{fig:comp2}
\end{figure}


\begin{itemize}
	\item Existing EFC methods are commonly trained using rudimentary image/class name signals, leading to the absence of rich semantic priors and distinct references.
	\item While the recent surge in Large-scale Language Models (LLMs)~\cite{devlin2018bert,brown2020language} has been instrumental in advancing multi-modal learning, primarily due to their impressive few-shot learning capabilities, CAC research has not yet utilized these models for enhancing zero-shot learning capability.
	\item Initial EFC approaches tend to extract exemplar cues by scanning the entire input image, a process that is both resource-intensive and less adept at quickly identifying locational hints. Conversely, as noted by Dehaene~\cite{dehaene2011number}, humans typically ``Receive-Parse-Comprehend" linguistic instructions before embarking on tasks such as subitizing or counting, see Figure~\ref{fig:comp2}.
\end{itemize}


%our goal is to remodel the exemplar-free counting problem as the perception-counting agent excelling in comprehending language-visual signals.

To remedy these deficiencies, a novel linguistic CAC architecture, namely Expression Counting Network \emph{(ExpressCount)}, is proposed to steer zero-shot counting via referring expression comprehension; see Figure~\ref{fig:main}. We aspire to integrate EFC with human-like imitation and linguistic intuition. For instance, when presented with the phrase ``a basket of books on a table'', humans, leveraging their accumulated knowledge and priors, can effortlessly discern key cues, such as the semantic understanding of ``books in a basket'' and the anticipated location of ``books at the center of the table", even in the absence of a direct visual reference.

To achieve this, we introduce an innovative referring expression comprehension module to explore the linguistic impacts on the counting problems. Recognizing the lack of linguistic annotations, we augment the CAC-specific dateset, FSC-147~\cite{ranjan2021learning}, with fine-grained referring expressions using the pre-trained LLM GPT~\cite{openai2023gpt4} and the visual-language BLIP~\cite{li2022blip}. This enriched dataset, dubbed \emph{FSC-147-Express}, paves the way for the creation of linguistically-informed counting models.
%It worth noting that although ZSC~\cite{xu2023zero} and ClipCount~\cite{jiang2023clip} explore the usage of one-word class name (\eg ``book"), they treat name word as the auxiliary signal and focus on guiding the feature learning of raw input scene. 
%comprehend these language descriptions. To marry the model with the higher perception/zero-shot ability, we 
%After gathering the referring expression, we proceed to transmit knowledge from the pre-trained LLM-~\cite{devlin2018bert} and Large-scale Visual Model (LVM)~\cite{carion2020end} by fine-tuning their partial encoders. 

Leveraging robust priors, our ExpressCount excels in perceiving and regressing exemplar cues (bounding boxes of exemplar patches). Both the learned exemplar and the original image are then seamlessly integrated into our meticulously crafted sibling sub-network, facilitating zero-shot count inference. Comprehensive tests underscore the prowess of our proposed ExpressCount. It not only surpasses current EFC approaches in performance, but also competes effectively with exemplar-dependent counters. In summary, this work offers four distinct contributions:

% To better verify the language-visual counting models, we also extend the current FSC-147 dataset by providing fine-grained descriptions with prior knowledge from LLM for each samples. 


\begin{figure*}[h]
	\begin{center}
		\includegraphics[width=\linewidth]{main.jpg}
	\end{center} 
	\caption{The overall architecture of our proposed ExpressCount, which integrates the plug-and-play referring expression comprehension with visual counting tasks. Particularly, the linguistic module takes a referring expression as input, and proceeds to comprehend the language signals and to predict the exemplar cues. Subsequently, a sibling-like network is designed to ``extract-fuse-compare" representations from exemplar and raw images, and infer the counts with unseen classes.}
	\label{fig:main}
\end{figure*}



\begin{itemize}
	\item  \textbf{In use:} A novel \emph{ExpressCount} is presented to steer zero-shot object counting. Unlike the previous models, it directly infers exemplar cues by comprehending the fine-grained referring expression with lots of semantic priors. Apart from the language parsing module, the multi-modal integration and sibling-like cross-attention/matching learning are exploited to infer counts.    
	\item \textbf{Application Scope:} The proposed module embraces the merits of plug-and-play attribute and broad applicability. It can be easily deployed to any exemplar-unseen counting scenarios without further fine-tuning. More importantly, our language-centered attempts allow for sufficing the need of adopting the modern LLMs to guide the human-machine interactions.  
	\item \textbf{Performance:} Our ExpressCount surpasses all CAC approaches and acquires the state-of-the-art counting accuracy, and is even quantitatively on par with methods using user-provided exemplars. 
	\item \textbf{Dataset Extension:} The prevailing CAC-specific FSC-147 benchmark is advanced to blaze a trail for fine-tuning and testifying the modern linguistic counting models.
	%by generating fine-grained referring expressions for each samples. 
	
\end{itemize}



















==> sec/2_review.tex <==
\section{Related Work}
Vast CSC approaches~\cite{liang2023crowdclip,ranasinghe2023diffuse,song2021rethinking,li2018csrnet,khan2016deep,rahnemoonfar2017deep,bui2020vehicle} have been raised to count object instances with pre-specified categories. Although achieving impressive counting accuracy, their success takes root in the troublesome collection of abundant training samples for each class type, which hinders the real-world applicability of counting models. This observation stimulates increasing endeavors on CAC, which can be subdivided into three sub-fields: Exemplar-Reliant Counting (ERC), Implicit Exemplar Learning (IEL) and Generalized Exemplar Learning (GEL).

\paragraph{Exemplar-Reliant CAC:}
Perusing few-shot learning in ERC aims to cater for widespread applications of counting model with the goal of reducing the costs of collecting adequate samples for all classes. The pioneering few-shot GMN~\cite{lu2018class} reformulates the counting task as the learning of matching objects to mine the similarity across the whole image.  CFOCNet~\cite{yang2021class} and FAMNet~\cite{ranjan2021learning} further enhance the counters' capability of few-shot learning through features matching. Furthermore, FAMNet releases the first benchmark dataset (FSC-147) for validating  CAC methods, which is use in a series of new approaches (\eg CounTR~\cite{liu2022countr}, LOCA~\cite{djukic2022low}, SPDCN~\cite{lin2022scale}, BMNet~\cite{shi2022represent} and SAFECount~\cite{you2023few}). Albeit allowing for counting arbitrary categories, these methods inevitably introduce a new requirement on user-provided exemplar cues. 

\paragraph{Implicit Exemplar Learning:}
Fully zero-shot settings in CAC open up promising vistas towards higher generalization \& intellectualization abilities in the field of visual counting. The first attempt is RepRPN-Counter~\cite{ranjan2022exemplar} which focuses on capturing the salient object from the original scenes via a region proposal module. Simultaneously,  RCC~\cite{hobley2022learning} and GCNet~\cite{wang2023gcnet} try to devise learning blocks to suffice to locate repetitive patterns directly from input image in an implicit manner. More recently, CLIP-Count~\cite{jiang2023clip} achieves zero-shot counting on open-world object categories by feeding ``class name-image" pair into the large-scale pre-trained CLIP model~\cite{radford2021learning}. While those efforts enable to learn exemplar hint automatically, they fail to perform well when encountering the play-and-plug scenarios, thereby stymieing the flexibility of generalized counting models. 

\paragraph{Generalized Exemplar Learning:}
The protocol of explicit exemplar learning is drawing increasing attention thanks to the merit of its play-and-plug attribute. The latest ZSC~\cite{xu2023zero} leverages a text-conditional variational autoencoder (VAE) model on a close-set classes to explicitly predict the exemplar patches. In spite of the impressive progress, the time-consuming transversal algorithm is used to select optimized patches, which is detrimental to the model's deployment. In comparison, our ExpressCount possesses advantages of both higher-efficiency (\ie discarding traversal overheads) and strong interaction. Instead of relying on one-word class name in CLIP-Count and ZSC, we extensively explore the human-imitated expression comprehension imposed on counting problems to pave the way for adopting modern language-vision models into the counting tasks. Towards better validating impacts of natural language on counting models, we also release an extended version of FSC-147 with fine-grained referring expressions. Concurrent with our attempts,  FSC-147-D~\cite{amini2023open} presents textual descriptions with correction and adjustment on class names. However, we observe that adopting descriptions from FSC-147-D degenerates the performance than using the original class names in FSC-147. In contrast, we delicately annotate referring expression with fine-grained semantics for each image in FSC-147.


==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
